Machine-Learning Potentials Predict Orientation- and Mode-Dependent Fracture in Refractory Diborides

Fracture toughness ($K_\mathrm{Ic}$) and fracture strength ($\sigma_\mathrm{f}$) are key criteria in the selection and design of reliable ceramics. However, their experimental characterization remains challenging -- especially for ceramic thin films, where size and interfacial effects hinder accurate and reproducible measurements. Here, machine-learning interatomic potentials (MLIPs) trained on \textit{ab initio} datasets of single crystal models deformed up to fracture are used to characterize transgranular cleavage in pre-cracked ceramic diboride TMB$_2$ (TM = Ti, Zr, Hf) lattices through stress intensity factor ($K$)-controlled loading. Mode-I simulations performed across distinct crack geometries show that fracture is primarily driven by straight crack extension along the original plane. The corresponding macroscale fracture-initiation properties ($K_\mathrm{Ic} \approx 1.7$-2.9 MPa$\cdot\sqrt{\text{m}}$, $\sigma_\mathrm{f} \approx 1.6$-2.4 GPa) are extrapolated using established scaling laws. Considering TiB$_2$ as a representative system, additional simulations explore loading conditions ranging from pure Mode-I (opening) to Mode-II (sliding). TiB$_2$ models containing prismatic cracks exhibit their lowest fracture resistance under mixed-mode conditions, where the crack deflects onto pyramidal planes--as confirmed by nanoindentation tests on TiB$_2$(0001) thin films. This study establishes $K$-controlled, MLIP-based simulations as predictive tools for orientation- and mode-dependent fracture in ceramics. The approach is readily extendable to finite temperatures for evaluating fracture behavior under conditions relevant to refractory applications.

==> OLD-0,5-Pre_Crack.tex <==
\section{Cracked-plate lattice models for simulations of fracture}

\begin{figure*}[!h]
\centering
\includegraphics[width=1.0\textwidth]{Figures/Fig2_Orientation.png}
\caption{\footnotesize 
{\bf{Possible Mode-I loading geometries}} in the hexagonal $\alpha$-structured diborides (considering orthogonalized supercells). 
(a) (0001) crack surface with $[10\overline{1}0]$ (up, $Nr.1$) and $[\overline{1}2\overline{1}0]$ (down, $Nr.2$) crack-front directions. 
(b) $(\overline{1}2\overline{1}0)$ crack surface with $[10\overline{1}0]$ (up, $Nr.3$) and [0001] (down, $Nr.4$) crack-front directions. 
(c) $(10\overline{1}0)$ crack surface with [0001] (up, $Nr.5$) and $[\overline{1}2\overline{1}0]$ (down, $Nr.6$) crack-front directions.
}
\label{Geo}
\end{figure*}

The macroscale mechanical properties of diborides are calculated by $K$-controlled loading of lattice models containing an atomically sharp crack (cracked-plate model). In K-controlled simulations, the stress-intensity factor is incremented sequentially to identify stress conditions corresponding to the onset of crack growth (refs. Curtin review 2018, Sangiovanni polymorph competition).  
The calculations are repeated as a function of the plate area (A), so that the fracture initiation toughness and fracture initiation strength can be extrapolated at the macroscale limit by constitutive scaling relations, as done in Ref.~\cite{sangiovanni2024controlled}. The fracture-initiation strength and fracture-initiation toughness of a plate with area A correspond to the $K$ value for which the crack tip has advanced by two percent of the model width. 
Below, the crack plane and crack line of a supercell are indicated as ($hklm$)[$h$'$k$'$l$'$m$'], where $h$, $k$, $l$, and $m$ and their primes are crystallographic indexes of a hexagonal lattice.

Fig.~\ref{Geo} illustrates six crack geometries characterized by low-index planes and crack-line directions for hexagonal $\alpha$-structured TMB$_{2}$:s. 
Among them, the orientations $(\overline{1}2\overline{1}0)$-$[10\overline{1}0]$ and $(10\overline{1}0)$-$[\overline{1}2\overline{1}0]$ have the crack plane orthogonal to the [0001] axis. 
Thus, simulation results of fracture properties obtained for model $Nr.1$ and $Nr.2$ in Fig.~\ref{Geo} are of the highest relevance for comparison with experimental testing. Since the [0001] is the typical growth direction of TMB$_{2}$ thin-film coatings, experimental toughness measurements induce crack formation normal to the (0001) plane. 
%It is important to note that for MS simulations, which relies on energy minimization principles, the thickness of the structure does not affect the results. This observation is consistent with the findings of P.Andric and W.A.Curtin~\cite{andric2018atomistic}, and a systematic validation of this behavior is provided in \textcolor{violet}{the Supplementary Material}.
%When it comes to molecular dynamics simulations, the effect of thickness must be carefully considered, as it involves dynamic atomic motion and thermal fluctuations, making size effects more pronounced. 
%A thicker structure can better capture stress redistribution, dislocation interactions, and out-of-plane deformation, leading to more realistic fracture behavior. 
%However, increasing the thickness also drastically raises the computational cost, a detailed analysis of thickness effects in MD simulations is beyond the scope of this work and will not be discussed further.

%Moreover, before comparing mechanical properties and behavior, certain non-trivial aspects must be addressed to establish a general rule for all geometries.
%Furthermore, note that for models based on the $(0001)$ and $(10\overline{1}0)$ planes, the displaced atoms are entirely TM atoms, whereas for the $(\overline{1}2\overline{1}0)$ plane, the displacement involves a mixture of B and TM atoms. 
%Within a single plane, the two opening distances, such as $Nr.1$ and $Nr.2$, are equal. 
%However, due to differences in lattice parameters, the opening distances vary among different TMB$_{2}$ materials. 
%Similarly, when comparing different planes, even when only one TM layer is displaced, the opening distances, such as $Nr.1$ and $Nr.3$, also differ.
%A comprehensive comparison of lattice parameters and zero-Kelvin elastic constants, along with MLIP validation, will be presented in the following chapter.
%The predicted value ($K_{Ic}$ and $\sigma_{max}$) corresponds to the model with an infinite plane area ($K_{Ic}^{\infty}$ and $\sigma_{max}^{\infty}$) to account for size effects, details are provided in {\bf{Methods}}.

==> OLD-2-Comparison.tex <==
\section{Mode-I loading (crack opening): comparison of different TMB$_{2}$:s}

\begin{figure*}[!h]
\centering
\includegraphics[width=1.0\textwidth]{Figures/Fig3_FullModel.png}
\caption{\footnotesize 
{\bf{Bond breakage and volumetric strain distribution subject to Mode-I loading as a function of stress intensity:}} before, shortly after, and well after reaching the $K_{Ic}$ point for different crack surfaces: (a, b) (0001), (c, d) $(\overline{1}2\overline{1}0)$, and (e, f) $(10\overline{1}0)$ planes. 
The first bond breakage occurs along the TM--B bond in (a, b), while in the other cases, the initial crack propagates along B--B bonds.
The snapshots illustrate volumetric strain. 
For $K_{I}=0$, all atoms appear in gray, while under increasing tensile, stress-responsive atoms turn red.}
\label{Bond}
\end{figure*}

\begin{figure*}[!h]
\centering
\includegraphics[width=1.0\textwidth]{Figures/Fig4-Comparison.png}
\caption{\footnotesize 
{\bf{Comparison of converged fracture toughness values (a, $K_{Ic}^{\infty}$) and maximum strength (b, $\sigma_{max}^{\infty}$) during Mode-I loading}} among different TMB$_{2}$ compounds and geometries. 
TiB$_{2}$ is shown in teal, ZrB$_{2}$ in red, and HfB$_{2}$ in orange. 
The results are ordered counterclockwise from $Nr.1$ to $Nr.6$, as defined in Fig.~\ref{Geo}.
(c) Example of $Nr.1$ ((0001)$[10\overline{1}0]$) geometry of TiB$_{2}$, with increasing plane area from 800~nm$^{2}$ (top) to 9000~nm$^{2}$ (down). 
The zoomed-in screenshot shows the behavior immediately after reaching $K_{Ic}$, with the fracture phenomenon remaining similar.
}
\label{mode1comp}
\end{figure*}

\begin{table*}[!h]
\centering
\small
\caption{\footnotesize 
{\bf{Mode-I fracture toughness ($K_{Ic}^{\infty}$) and Griffith fracture toughness ($K_{Ic}^{G}$).}} 
The former is obtained from $K$-controlled static Mode-I simulations, while the latter is derived from unrelaxed surface energy ($E_{surf}^{un}$) in ML-MS calculations. 
Additionally, the converged maximum stress values ($\sigma_{max}^{\infty}$) are also compared. 
All converged values are presented with standard deviations, calculated as described in Ref.~\cite{sangiovanni2023descriptor}.}
\resizebox{\textwidth}{!}{
\begin{tabular}{ccccccccccccccccc}
    \hline
    \hline
    \footnotesize 
    Geometry & \multicolumn{3}{c}{TiB$_{2}$ }& \multicolumn{3}{c}{ZrB$_{2}$} & \multicolumn{3}{c}{HfB$_{2}$}\\
      { } & K$_{Ic}^{\infty}$ (MPa\cdot\sqrt{m}) & K$_{Ic}^{G}$ (MPa\cdot\sqrt{m}) & \sigma$_{max}^{\infty}$ (GPa) & K$_{Ic}^{\infty}$ (MPa\cdot\sqrt{m}) & K$_{Ic}^{G}$ (MPa\cdot\sqrt{m}) & \sigma$_{max}^{\infty}$ (GPa) & K$_{Ic}^{\infty}$ (MPa\cdot\sqrt{m}) & K$_{Ic}^{G}$ (MPa\cdot\sqrt{m}) & \sigma$_{max}^{\infty}$ (GPa)  \\
    \hline
    {$(0001)$$[10\overline{1}0]$ ($Nr.1$)} & {1.81 $\pm$ 0.03}  & {2.02} & {2.00 $\pm$ 0.77} & {2.03 $\pm$ 0.04} & {1.86} & {1.83 $\pm$ 0.65} & {2.75 $\pm$ 0.02} & {1.93} & {2.02 $\pm$ 0.64}\\
    {$(0001)$$[\overline{1}2\overline{1}0]$ ($Nr.2$)} & {2.35 $\pm$ 0.03}  & { 2.20} & {1.97 $\pm$ 0.49} & {2.08 $\pm$ 0.02} & {1.98} & {1.89 $\pm$ 0.22} & {2.89 $\pm$ 0.02} & {2.05} & {2.04 $\pm$ 0.31}\\
    {$(0001)$} & \multicolumn{3}{c}{$E_{surf}^{un}$: 4.02 (J/m$^{2}$)} & \multicolumn{3}{c}{$E_{surf}^{un}$: 3.68 (J/m$^{2}$)} & \multicolumn{3}{c}{$E_{surf}^{un}$: 3.61 (J/m$^{2}$)}\\
    \hline
    {$(\overline{1}2\overline{1}0)$$[10\overline{1}0]$ ($Nr.3$)} & {2.24 $\pm$ 0.02}  & {2.37} & {2.24 $\pm$ 0.63} & {1.74 $\pm$ 0.02 } & {2.18} & {2.21 $\pm$ 0.68} & {2.01 $\pm$ 0.02} & {2.20} & {2.27 $\pm$ 0.61} \\
    {$(\overline{1}2\overline{1}0)$$[0001]$ ($Nr.4$)} & {1.88 $\pm$ 0.02}  & { 2.29} & {2.22 $\pm$ 0.67} & {1.84 $\pm$ 0.02} & {2.15} & {1.75 $\pm$ 0.29} & {2.25 $\pm$ 0.05} & {2.18} & {1.61 $\pm$ 0.54}\\
    {$(\overline{1}2\overline{1}0)$} & \multicolumn{3}{c}{$E_{surf}^{un}$: 4.36 (J/m$^{2}$)} & \multicolumn{3}{c}{$E_{surf}^{un}$: 4.33 (J/m$^{2}$)} & \multicolumn{3}{c}{$E_{surf}^{un}$: 4.07 (J/m$^{2}$)}\\    
    \hline
    {$(10\overline{1}0)$$[0001]$ ($Nr.5$)} & {2.25 $\pm$ 0.02}  & {2.24} & {2.26 $\pm$ 0.69} & {1.74 $\pm$ 0.02} & {2.04} & {2.21 $\pm$ 0.68} & {2.74 $\pm$ 0.03} & {2.22} & {2.36 $\pm$ 0.47} \\
    {$(10\overline{1}0)$$[\overline{1}2\overline{1}0]$ ($Nr.6$)} & {2.24 $\pm$ 0.02}  & {2.16} & {1.97 $\pm$ 0.60} & {1.93 $\pm$ 0.02} & {2.01} & {2.11 $\pm$ 0.33} & {2.25 $\pm$ 0.02} & {2.20} & {2.26 $\pm$ 0.34}\\
    {$(10\overline{1}0)$} & \multicolumn{3}{c}{$E_{surf}^{un}$: 3.88 (J/m$^{2}$)} & \multicolumn{3}{c}{$E_{surf}^{un}$: 3.81 (J/m$^{2}$)} & \multicolumn{3}{c}{$E_{surf}^{un}$: 4.15 (J/m$^{2}$)}\\
\hline
\hline
\end{tabular}
}
\label{Comp}
\end{table*}

K-controlled simulations are carried out at 0 K, using our MLIPs in a MS framework. The mechanical behaviors of TMB$_{2}$ at different stages of pure Mode-I loading are shown in Fig.~\ref{Bond}, where the definition of crack-plane and crack-line directions is consistent with Fig.~\ref{Geo}. 
The figure visualizes atomic configurations at $K_{I}$ values preceding, immediately after, and far beyond the onset of crack growth.

For geometries based on the $(0001)$ plane (Fig.~\ref{Geo}-(a)), the B--TM bonds consistently break first, while for those based on the $(\overline{1}2\overline{1}0)$ (Fig.~\ref{Geo}-(b)) and $(10\overline{1}0)$ (Fig.~\ref{Geo}-(c)) planes, the B--B bonds are the first to break. 
During the Mode-I opening process, as $K_{I}$ increases ($K_{I}\leq K_{Ic}$), stress becomes increasingly concentrated at the atom located at the crack tip. 
Upon reaching $K_{Ic}$, the corresponding bond breaks. 
Typically, only one bond breaks at this stage, but simultaneous breaking of multiple bonds is also possible, as observed in $Nr.3$ (Fig.~\ref{Bond}-(c)).
Beyond this point, as $K_{I}$ increases further ($K_{I}\gg K_{Ic}$), the crack propagates in a certain direction, typically along the crack plane ($Nr.1$:  Fig.~\ref{Bond}-(a); $Nr.3$: Fig.~\ref{Bond}-(c); $Nr.4$: Fig.~\ref{Bond}-(d)).
The crack propagation, however, may be more complicated, e.g., following a zigzag pattern ($Nr.2$: Fig.~\ref{Bond}-(b); $Nr.5$: Fig.~\ref{Bond}-(e)), or growing diagonally across the lattice ($Nr.6$.: Fig.~\ref{Bond}-(f)).
The detailed mechanisms underlying these propagation behaviors will be analyzed below.

Fig.~\ref{mode1comp} compares $K_{Ic}^{\infty}$ (Fig.~\ref{mode1comp}-(a)) and $\sigma_{max}^{\infty}$ (Fig.~\ref{mode1comp}-(b)) for the Group-IV TMB$_{2}$:s, derived as extrapolative values for an infinite plate area.
Following Ref.~\cite{sangiovanni2023descriptor}, the data is fitted using a combined inverse polynomial function against the plate area ($L^{2}$)~\cite{sangiovanni2024controlled}, as further detailed in \textcolor{black}{the supplementary material}.
Overall, HfB$_{2}$ exhibits the highest $K_{Ic}^{\infty}$ (mainly $\approx$2.8~MPa$\cdot\sqrt{m}$), except for $Nr.3$ (TiB$_{2}$ is the highest with 2.24~MPa$\cdot\sqrt{m}$, whereas HfB$_{2}$ has 2.01~MPa$\cdot\sqrt{m}$), while ZrB$_{2}$ shows the lowest (mainly $\approx$1.8~MPa$\cdot\sqrt{m}$), except for $Nr.1$ (TiB$_{2}$ is the lowest with 1.81~MPa$\cdot\sqrt{m}$, whereas ZrB$_{2}$ has 2.03~MPa$\cdot\sqrt{m}$). 
In terms of $\sigma_{max}^{\infty}$, the three materials display similar values (mainly $\approx$2.0~GPa), with the notable exception of $Nr.4$, where TiB$_{2}$ demonstrates significantly higher values (TiB$_{2}$ remains $\approx$2.0~GPa, where the others have $\approx$1.7~GPa). 
%This behavior is consistent with the highest tensile strength observed along the [$\overline{1}2\overline{1}0$] direction (Fig.~\ref{Vali}-(a)).
Contrarily to strongly size-dependent fracture mechanisms and nearly size-independent strength subject to uniaxial tensile tests for single crystals~\cite{lin2024machine}, Mode-I opening simulations reveal significant size effects in both strength and $K_{Ic}$. 
However, the crack growth mechanisms remain very similar for TM$=$Ti, Zr, Hf (Fig.~\ref{mode1comp}-(c)) and are almost independent of the plate size. 
%With increasing plate sizes, both $K_{Ic}$ and $\sigma_{max}$ decrease asymptotically, yet the crack opening behavior right after reaching $K_{Ic}$ remains qualitatively similar.
%The extrapolated values ($\sigma_{max}^{\infty}$ and $K_{Ic}^{\infty}$) for an infinite plane area are shown in Fig.~\ref{mode1comp}. 

Tab.~\ref{Comp} lists the predicted $K_{Ic}$s---precisely, the infinite-plate-extrapolation values, $K_{Ic}^{\infty}$---together with the Griffith's $K_{Ic}^{G}$ estimates derived from the surface energy and zero-Kelvin elastic constants (Tab.~\ref{SE}).
Note that $K_{Ic}^{G}$ considers ideal fracture surface parallel to the pre-crack~\cite{brace1960extension}, which does not fully capture the fracture behavior observed in our $K$-controlled simulations.  
Overall, the difference between $K_{Ic}^{\infty}$ and $K_{Ic}^{G}$ falls within the range of 0.5--20\%, with the exception of $Nr.1$ and $Nr.2$ for HfB$_{2}$, where $K_{Ic}^{G}$ is approximately 30\% lower than $K_{Ic}^{\infty}$. 
Additional data is provided in the \textcolor{black}{the supplementary material}.

During pure Mode-I opening, Group-IV TMB$_{2}$ materials exhibit similar behavior, as illustrated in Fig.~\ref{mode1para}, with one representative example for each plane ($Nr.1$: Fig.~\ref{mode1para}-(a), $Nr.3$: Fig.~\ref{mode1para}-(b), $Nr.6$: in Fig.~\ref{mode1para}-(c)). 
For $Nr.1$--$Nr.4$, the first TM--B bond breaks upon reaching the $K_{Ic}$ point (as shown in the sub-patterns in each row and Fig.~\ref{Bond}-(a-d)), and the opening continues along the corresponding plane: (0001) for $Nr.1$ and $Nr.2$ (zigzag path), and $(\overline{1}2\overline{1}0)$ for $Nr.3$ and $Nr.4$. 
Contrarily for the $(10\overline{1}0)$ plane, differences arise from the bond-breaking sequence after the initial B--B bond breaks at $K_{Ic}$ (as shown in the sub-patterns and Fig.~\ref{Bond}-e,f).
In all Group-IV TMB$_{2}$ compounds, the crack tip advances primarily through the continuous breaking of TM--B bonds, as B--B bonds are generally much stronger than TM--B bonds in $\alpha$-structured TMB$_{2}$ compounds~\cite{zhou2015general}. 
The difference lies in the propagation patterns: in TiB$_{2}$, the breaking sequence forms a zigzag path but remains along the horizontal direction (Fig.~\ref{mode1para}-(c-1)), whereas in ZrB$_{2}$ and HfB$_{2}$, the crack tip advances diagonally along the $(1\overline{1}01)$ plane (Fig.~\ref{mode1para}-(c-2,3)).
Importantly, despite the predominant crack opening in TiB$_2$ occurs along the $(10\overline{1}0)$ plane, the actual fracture surface is more complex than that assumed by the Griffith's theory, which would disregard the alternations between mirrored diagonal facets.
The observed difference in crack propagation patterns may be attributed to the small differences between $(10\overline{1}0)$ and $(1\overline{1}01)$ surface energies.
%which corresponds to the first pyramidal plane and represents the preferred fracture surface, as previous shown for TiB$_{2}$~\cite{lin2024machine}.
%Notably, this diagonal surface also becomes the primary fracture path in TiB$_{2}$ when mixed with a small percentage of Mode-II shearing. 
%This phenomenon will be further discussed in the context of Mode-II deformation in the following section.


\begin{figure}[!h]
\centering
\includegraphics[width=0.5\textwidth]{Figures/Fig5_Ti-Zr-Hf.png}
\caption{\footnotesize 
{\bf{Comparison of fracture mechanisms after reaching $K_{Ic}$}} for the studied TMB$_{2}$:s, with one example from each crack surface: 
(a) (0001)$[10\overline{1}0]$ ($Nr.1$) for the (0001) plane, (b) $(\overline{1}2\overline{1}0)$$[10\overline{1}0]$ ($Nr.3$) for the $(\overline{1}2\overline{1}0)$ plane, and (c) $(10\overline{1}0)$$[\overline{1}2\overline{1}0]$ ($Nr.6$) for the $(10\overline{1}0)$ plane. 
Mode-I loading results are shown for TiB$_{2}$ (*-1), ZrB$_{2}$ (*-2), and HfB$_{2}$ (*-3). 
Small, zoomed-in snapshots depict the state shortly after reaching $K_{Ic}$ ($K_{I}$=$K_{Ic}+0.02$,i.e., one step further), while larger, overall snapshots illustrate the fracture behavior well beyond $K_{Ic}$ ($K_{I}>K_{Ic}+0.50$).
The dark gray atoms represent metal (TM$=$Ti, Zr, Hf), as the blue atoms for boron.
Plate area of the selected model is $L^{2}\approx{30\times30}=900~\text{nm}^{2}$.
}
\label{mode1para}
\end{figure}

% TiB2: 3.8 or 6.0~\cite{ferber1983effect}, 1.8~\cite{bhaumik2000synthesis}, 4.1-6.8~\cite{wang2002influence}
% ZrB2: 2.2-4.7~\cite{monteverde2003advances}, 3.1-4.1~\cite{csanadi2024effect},3.2-5.0~\cite{swab2023mechanical}
% HfB2: 4.0-7.2~\cite{li2024synthesis}, 2.8-3.5~\cite{wang2015fabrication}

The fracture toughness from experiment ranges between 1.8--6.8~MPa$\sqrt{m}$ for TiB$_2$~\cite{ferber1983effect,bhaumik2000synthesis,wang2002influence}, 2.2--5.0~MPa$\sqrt{m}$ for ZrB$_2$~\cite{monteverde2003advances,csanadi2024effect,swab2023mechanical}, and 2.8--7.2~MPa$\sqrt{m}$ for HfB$_2$~\cite{li2024synthesis,wang2015fabrication}. 
These values align with ML-MS predictions in Fig.~\ref{mode1comp} and Tab.~\ref{Comp}, where the differences between our data and data from various experimental studies (note the significant spread in experimental values) stem from various sample preparation methods, microstructural effects, as well as particular mechanical testing approach.
Furthermore, the possibility of mixing with Mode-II shearing or the Mode-III tearing introduces variations in the experimentally obtained $K_{Ic}$s. 
While Mode-III is rather exotic for brittle materials~\cite{maccagno1985brittle}, hence disregarded in this work, mixed Mode-I and Mode-II effects are explored in the following section. 

%While we aim for a fair comparison, these differences introduce uncertainties, and the experimental data should be interpreted as a reference for a general overview rather than an absolute benchmark.


Fig.~\ref{mode1para} compares fracture mechanisms of TiB$_2$, Zr$_2$, and HfB$_2$ after reaching $K_{Ic}$, considering the most experimentally relevant (0001)$[10\overline{1}0]$ ($Nr.1$), $(\overline{1}2\overline{1}0)$$[10\overline{1}0]$ ($Nr.3$), and  $(10\overline{1}0)$$[\overline{1}2\overline{1}0]$ ($Nr.6$) crack geometries. 
Among them, only the opening in the $Nr.3$ geometry (Fig.~\ref{mode1para}-(b)) shows that each TMB$_{2}$ compound breaks the same number of bonds. 
For the other two geometries, $Nr.1$ (Fig.~\ref{mode1para}-(a)) and $Nr.6$ (Fig.~\ref{mode1para}-(c)), TiB$_{2}$ consistently breaks a single bond, while ZrB$_{2}$ and HfB$_{2}$ rupture multiple bonds simultaneously.
This suggests that stress in ZrB$_{2}$ and HfB$_{2}$ redistributes more effectively, leading to abrupt fracture.
Despite their high $G/B$ values among all TMB$_{2}$:s---indicating intrinsic brittleness~\cite{zhou2014first,zhou2015general}---variations in crack-tip shielding, bond anisotropy, or localized deformation mechanisms further influence the fracture behavior.
